Anchored Alignment: Preventing Positional Collapse in Multimodal Recommender Systems

Multimodal recommender systems (MMRS) leverage images, text, and interaction signals to enrich item representations. However, recent alignment based MMRSs that enforce a unified embedding space often blur modality specific structures and exacerbate ID dominance. Therefore, we propose AnchorRec, a multimodal recommendation framework that performs indirect, anchor based alignment in a lightweight projection domain. By decoupling alignment from representation learning, AnchorRec preserves each modality's native structure while maintaining cross modal consistency and avoiding positional collapse. Experiments on four Amazon datasets show that AnchorRec achieves competitive top N recommendation accuracy, while qualitative analyses demonstrate improved multimodal expressiveness and coherence. The codebase of AnchorRec is available at https://github.com/hun9008/AnchorRec.

==> Plot/plot-eq5-all.tex <==
\begin{figure}[!t]  

\small
\begin{tikzpicture}
\begin{groupplot}[
  group style={
    group size=3 by 1,
    horizontal sep=18pt,
    vertical sep=22pt,               % ★ 행 사이 여백 (8–12pt 사이에서 조정)
    xlabels at=edge bottom,
    ylabels at=edge left,
    xticklabels at=edge bottom
  },
  width=3.5cm, height=2.8cm,
  ylabel={Recall@10},
  ymajorgrids=true,
  every axis/.append style={axis line style, trim axis left},
  every axis y label/.style={
    at={(axis description cs:-0.3,0.5)},  % y라벨을 왼쪽 바깥으로 고정
    anchor=south, rotate=90, outer sep=0pt
  },
  y tick scale label style={yshift=-1pt},
]

% ===== Row 1: Wikipedia =====
% (a) alpha_user
\nextgroupplot[xlabel={(a) $\alpha_{\text{user}}$}, ymin=0.2, ymax=0.35]
  \addplot[color=blue, mark=*, dashed] coordinates {
    (5,0.2922) (10,0.2911) (15,0.2973) (20,0.2887) (25,0.2947)
    (30,0.2955) (35,0.2947) (40,0.2952) (45,0.2921) (50,0.2889)
  };

% (b) alpha_item
\nextgroupplot[xlabel={(b) $\alpha_{\text{item}}$},  ymin=0.2, ymax=0.35]
  \addplot[color=orange, mark=*, dashed] coordinates {
    (5,0.2918) (10,0.2952) (15,0.2973) (20,0.2948) (25,0.2961)
    (30,0.2944) (35,0.2965) (40,0.2900) (45,0.2912) (50,0.2842)
  };

% (c) beta
\nextgroupplot[xlabel={(c) $\beta$}, xtick={1,2,3,4}, ymin=0.2, ymax=0.35]
   \addplot[color=darkgreen, mark=*, dashed] coordinates {(1,0.2864) (2,0.2973) (3,0.2948) (4,0.2907)};% lastFM
\end{groupplot}
\node[font=\bfseries, yshift=5pt, anchor=south]
  at ($(group c1r1.north)!0.5!(group c3r1.north)$) {LastFM};
\end{tikzpicture}
\normalsize


%MOOC

\small
\begin{tikzpicture}
\begin{groupplot}[
  group style={
    group size=3 by 1,
    horizontal sep=18pt,
    vertical sep=22pt,               % ★ 행 사이 여백 (8–12pt 사이에서 조정)
    xlabels at=edge bottom,
    ylabels at=edge left,
    xticklabels at=edge bottom
  },
  width=3.5cm, height=2.8cm,
  ylabel={Recall@10},
  ymajorgrids=true,
  every axis/.append style={axis line style, trim axis left},
  every axis y label/.style={
    at={(axis description cs:-0.3,0.5)},  % y라벨을 왼쪽 바깥으로 고정
    anchor=south, rotate=90, outer sep=0pt
  },
  y tick scale label style={yshift=-1pt},
]

% ===== Row 1: MOOC =====
% (a) alpha_user
\nextgroupplot[xlabel={(a) $\alpha_{\text{user}}$},  ymin=0.7, ymax=0.85]
  \addplot[color=blue, mark=*, dashed] coordinates {
    (5,0.7735) (10,0.7752) (15,0.7670) (20,0.7716) (25,0.7728)
    (30,0.7771) (35,0.7871) (40,0.7752) (45,0.7681) (50,0.771)
  };

% (b) alpha_item
\nextgroupplot[xlabel={(b) $\alpha_{\text{item}}$},   ymin=0.7, ymax=0.85]
  \addplot[color=orange, mark=*, dashed] coordinates {
    (5,0.7461) (10,0.7369) (15,0.7757) (20,0.7871) (25,0.7789)
    (30,0.7731) (35,0.7732) (40,0.7820) (45,0.7727) (50,0.7751)
  };

% (c) beta
\nextgroupplot[xlabel={(c) $\beta$}, xtick={1,2,3,4},  ymin=0.7, ymax=0.85]
   \addplot[color=darkgreen, mark=*, dashed] coordinates {(1,0.7762) (2,0.7871) (3,0.775) (4,0.7751)}; % MOOC
\end{groupplot}
\node[font=\bfseries, yshift=5pt, anchor=south]
  at ($(group c1r1.north)!0.5!(group c3r1.north)$) {MOOC};
\end{tikzpicture}
\normalsize


%WIKI

\small
\begin{tikzpicture}
\begin{groupplot}[
  group style={
    group size=3 by 1,
    horizontal sep=18pt,
    vertical sep=22pt,               % ★ 행 사이 여백 (8–12pt 사이에서 조정)
    xlabels at=edge bottom,
    ylabels at=edge left,
    xticklabels at=edge bottom
  },
  width=3.5cm, height=2.8cm,
  ylabel={Recall@10},
  ymajorgrids=true,
  every axis/.append style={axis line style, trim axis left},
  every axis y label/.style={
    at={(axis description cs:-0.3,0.5)},  % y라벨을 왼쪽 바깥으로 고정
    anchor=south, rotate=90, outer sep=0pt
  },
  y tick scale label style={yshift=-1pt},
]

% ===== Row 1: Wikipedia =====
% (a) alpha_user
\nextgroupplot[xlabel={(a) $\alpha_{\text{user}}$}, ymin=0.5, ymax=0.85]
  \addplot[color=blue, mark=*, dashed] coordinates {
    (5,0.7409) (10,0.7779) (15,0.7472) (20,0.7732) (25,0.7711)
    (30,0.7731) (35,0.7461) (40,0.6570) (45,0.6948) (50,0.6625)
  };

% (b) alpha_item
\nextgroupplot[xlabel={(b) $\alpha_{\text{item}}$}, ymin=0.5, ymax=0.85]
  \addplot[color=orange, mark=*, dashed] coordinates {
    (5,0.7038) (10,0.7495) (15,0.7750) (20,0.7736) (25,0.7068)
    (30,0.7720) (35,0.7410) (40,0.7731) (45,0.7779) (50,0.7233)
  };

% (c) beta
\nextgroupplot[xlabel={(c) $\beta$}, xtick={1,2,3,4}, ymin=0.5, ymax=0.85]
  \addplot[color=darkgreen, mark=*, dashed] coordinates {(1,0.777) (2,0.7779) (3,0.7563) (4,0.6171)}; %wiki


\end{groupplot}

\node[font=\bfseries, yshift=5pt, anchor=south]
  at ($(group c1r1.north)!0.5!(group c3r1.north)$) {Wikipedia};

\end{tikzpicture}
\normalsize

% Yoochoose
\small
\begin{tikzpicture}
\begin{groupplot}[
  group style={
    group size=3 by 1,
    horizontal sep=18pt,
    vertical sep=22pt,               % ★ 행 사이 여백 (8–12pt 사이에서 조정)
    xlabels at=edge bottom,
    ylabels at=edge left,
    xticklabels at=edge bottom
  },
  width=3.5cm, height=2.8cm,
  ylabel={Recall@10},
  ymajorgrids=true,
  every axis/.append style={axis line style, trim axis left},
  every axis y label/.style={
    at={(axis description cs:-0.3,0.5)},  % y라벨을 왼쪽 바깥으로 고정
    anchor=south, rotate=90, outer sep=0pt
  },
  y tick scale label style={yshift=-1pt},
]

% ===== Row 1: Yoochoose =====
% (a) alpha_user
\nextgroupplot[xlabel={(a) $\alpha_{\text{user}}$}, ymin=0.02, ymax=0.04]
  \addplot[color=blue, mark=*, dashed] coordinates  {
    (5,0.0332) (10,0.0319) (15,0.0318) (20,0.0355) (25,0.0324)
    (30,0.0329) (35,0.0331) (40,0.0332) (45,0.0333) (50,0.0334)
  }; %Yoochoose

% (b) alpha_item
\nextgroupplot[xlabel={(b) $\alpha_{\text{item}}$}, ymin=0.02, ymax=0.04]
  \addplot[color=orange, mark=*, dashed] coordinates {
    (5,0.0355) (10,0.0323) (15,0.0331) (20,0.0316) (25,0.0325)
    (30,0.0323) (35,0.0323) (40,0.0327) (45,0.0325) (50,0.0319)
  }; %Yoochoose

% (c) beta
\nextgroupplot[xlabel={(c) $\beta$}, xtick={1,2,3,4}, ymin=0.02, ymax=0.04]
  \addplot[color=darkgreen, mark=*, dashed] coordinates {(1,0.0336) (2,0.0355) (3,0.0337) (4,0.0336)}; %Yoochoose

\end{groupplot}

\node[font=\bfseries, yshift=5pt, anchor=south]
  at ($(group c1r1.north)!0.5!(group c3r1.north)$) {Yoochoose};

\end{tikzpicture}
\normalsize



% Douban
\small
\begin{tikzpicture}
\begin{groupplot}[
  group style={
    group size=3 by 1,
    horizontal sep=18pt,
    vertical sep=22pt,               % 행 사이 여백 (8–12pt 사이에서 조정)
    xlabels at=edge bottom,
    ylabels at=edge left,
    xticklabels at=edge bottom
  },
  width=3.5cm, height=2.8cm,
  ylabel={Recall@10},
  ymajorgrids=true,
  every axis/.append style={axis line style, trim axis left},
  every axis y label/.style={
    at={(axis description cs:-0.3,0.5)},  % y라벨을 왼쪽 바깥으로 고정
    anchor=south, rotate=90, outer sep=0pt
  },
  y tick scale label style={yshift=-1pt},
]

% ===== Row 1: Douban =====
% (a) alpha_user
\nextgroupplot[xlabel={(a) $\alpha_{\text{user}}$}, ymin=0.0, ymax=0.02]
  \addplot[color=blue, mark=*, dashed] coordinates {
    (5,0.0099) (10,0.0103) (15,0.0099) (20,0.0102) (25,0.0091)
    (30,0.0094) (35,0.0099) (40,0.0103) (45,0.0094) (50,0.0094)
  };%Douban

% (b) alpha_item
\nextgroupplot[xlabel={(b) $\alpha_{\text{item}}$}, ymin=0, ymax=0.02]
  \addplot[color=orange, mark=*, dashed] coordinates {
    (5,0.0095) (10,0.0102) (15,0.0103) (20,0.0103) (25,0.0103)
    (30,0.0103) (35,0.0103) (40,0.0090) (45,0.0089) (50,0.0088)
  }; %Douban

% (c) beta
\nextgroupplot[xlabel={(c) $\beta$}, xtick={1,2,3,4},ymin=0, ymax=0.02]
  \addplot[color=darkgreen, mark=*, dashed] coordinates {(1,0.0094) (2,0.0103) (3,0.0088) (4,0.0096)}; %Douban

\end{groupplot}

\node[font=\bfseries, yshift=5pt, anchor=south]
  at ($(group c1r1.north)!0.5!(group c3r1.north)$) {Douban Movie};

\end{tikzpicture}
\normalsize


% VIDEO
\small
\begin{tikzpicture}
\begin{groupplot}[
  group style={
    group size=3 by 1,
    horizontal sep=18pt,
    vertical sep=22pt,               %  행 사이 여백 (8–12pt 사이에서 조정)
    xlabels at=edge bottom,
    ylabels at=edge left,
    xticklabels at=edge bottom
  },
  width=3.5cm, height=2.8cm,
  ylabel={Recall@10},
  ymajorgrids=true,
  every axis/.append style={axis line style, trim axis left},
  every axis y label/.style={
    at={(axis description cs:-0.3,0.5)},  % y라벨을 왼쪽 바깥으로 고정
    anchor=south, rotate=90, outer sep=0pt
  },
  y tick scale label style={yshift=-1pt},
]

% ===== Row 1: video =====
% (a) alpha_user
\nextgroupplot[xlabel={(a) $\alpha_{\text{user}}$}, ymin=0.02, ymax=0.08]
  \addplot[color=blue, mark=*, dashed] coordinates  {
    (5,0.0611) (10,0.0619) (15,0.0621) (20,0.0700) (25,0.0636)
    (30,0.0576) (35,0.0584) (40,0.0644) (45,0.063) (50,0.0584)
  };%video

% (b) alpha_item
\nextgroupplot[xlabel={(b) $\alpha_{\text{item}}$}, ymin=0.02, ymax=0.08]
  \addplot[color=orange, mark=*, dashed] coordinates  {
    (5,0.0619) (10,0.0644) (15,0.0700) (20, 0.0641) (25, 0.0638)
    (30,0.0563) (35,0.0609) (40,0.0614) (45,0.0584) (50,0.0606)
  }; %video

% (c) beta
\nextgroupplot[xlabel={(c) $\beta$}, xtick={1,2,3,4}, ymin=0.02, ymax=0.08]
  \addplot[color=darkgreen, mark=*, dashed] coordinates {(1,0.0574) (2,0.0706) (3,0.0595) (4,0.0636)}; %video

\end{groupplot}

\node[font=\bfseries, yshift=5pt, anchor=south]
  at ($(group c1r1.north)!0.5!(group c3r1.north)$) {Amazon-Video};

\end{tikzpicture}
\normalsize
\caption{Hyperparameter sensitivity in {\ours}.
} \label{plot:eq5-all}

\vspace{-2mm}
\end{figure}
